Machine-learned molecular mechanics force field for the simulation of protein-ligand systems and beyond

The development of reliable and extensible molecular mechanics (MM) force fields -- fast, empirical models characterizing the potential energy surface of molecular systems -- is indispensable for biomolecular simulation and computer-aided drug design. Here, we introduce a generalized and extensible machine-learned MM force field, \texttt{espaloma-0.3}, and an end-to-end differentiable framework using graph neural networks to overcome the limitations of traditional rule-based methods. Trained in a single GPU-day to fit a large and diverse quantum chemical dataset of over 1.1M energy and force calculations, \texttt{espaloma-0.3} reproduces quantum chemical energetic properties of chemical domains highly relevant to drug discovery, including small molecules, peptides, and nucleic acids. Moreover, this force field maintains the quantum chemical energy-minimized geometries of small molecules and preserves the condensed phase properties of peptides, self-consistently parametrizing proteins and ligands to produce stable simulations leading to highly accurate predictions of binding free energies. This methodology demonstrates significant promise as a path forward for systematically building more accurate force fields that are easily extensible to new chemical domains of interest.

==> figures/fig_optimize.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.8\textwidth]{figures/optimize.png}
    \caption{
    \textbf{Espaloma-derived molecular mechanics force fields preserve the location of quantum chemical energy minima.} 
    Kernel density estimate (KDE) plot (upper) and empirical cumulative density function (CDF) of aligned root mean square deviation (RMSD) between quantum chemical minima and MM-optimized minima using parameters from either \texttt{espaloma-0.3} or other well-estabilished force fields for small molecules. The superposed structures of the QM-minima (gold) and MM-optimized minima (cyan) are depicted in the KDE plot, showing the minimum, median, and maximum RMSDs.
    This qualitative experiment shows that the energy minima determined by \texttt{espaloma-0.3} is close to the quantum chemical energy minima.
    }
    \label{fig:optimize}
\end{figure}

==> leave_out_rmse.tex <==

% leave out QM data subset and QCArchive workflow experiment
\input{figures/fig_leave_out.tex}

\section{Chemical diversity and high-energy conformers are important for accurately capturing quantum chemical energies and forces with Espaloma}
\label{sec:leaveout}
To evaluate how each dataset used to train \texttt{espaloma-0.3} affects the reproducibility of quantum chemical energetic properties, we conducted a cross-validation experiment where we excluded either certain categories from chemical species (small molecules, peptides, or RNA) or dataset classes (single-point energies generated by MD [\texttt{Dataset}], optimization trajectories of enumerated conformers [\texttt{OptimizationDataset}], or one-dimensional torsion drives [\texttt{TorsionDriveDataset}]) from the training process ({\bf Figure~\ref{fig:leave_out}}). 

The quantum chemical forces for small molecules (non-biopolymer molecules) are poorly reproduced when small molecules were all excluded from the training such that only peptides and nucleic acids remain ({\bf Figure~\ref{fig:leave_out} (a)}). However, the quantum chemical energies were well-reproduced for most small molecule datasets, except for the \texttt{SPICE-Pubchem} dataset. 
The \texttt{SPICE-Pubchem} dataset is expected to be more difficult to capture the quantum chemical energy surfaces than the other small molecule datasets since it is much larger and chemically diverse. 
For peptides and RNA molecules, both the quantum chemical energies and forces of these molecules were well reproduced even when these molecules were excluded from the training dataset. 
This suggests that training on diverse datasets with broad chemical coverage---namely the \texttt{SPICE-Pubchem} dataset---is important to perceive and extrapolate the chemical environments for out-of-distributed chemical domain.

Interestingly, the quantum chemical forces of \texttt{SPICE-Pubchem} (small molecules) and \texttt{SPICE-Dipeptide} (peptides) were poorly reproduced when the datasets from the QCArchive \texttt{Dataset} workflow (which stores relatively high energy conformers) were excluded from the training process ({\bf Figure~\ref{fig:leave_out} (b)}). This is despite the fact that the small molecules and peptides from a different QCArchive workflow (\texttt{OptimizationDataset} and \texttt{TorsionDriveDataset}), which includes local energy minima conformers, were included in the training. 
We therefore hypothesize that high-energy conformers may be important to accurately capture the quantum chemical energies and forces with Espaloma. 


